Transformer-based GAN for Terahertz Spatial-Temporal Channel Modeling and Generating

Terahertz (THz) communications are envisioned as a promising technology for 6G and beyond wireless systems, providing ultra-broad continuous bandwidth and thus Terabit-per-second (Tbps) data rates. However, as foundation of designing THz communications, channel modeling and characterization are fundamental to scrutinize the potential of the new spectrum. Relied on time-consuming and costly physical measurements, traditional statistical channel modeling methods suffer from the problem of low accuracy with the assumed certain distributions and empirical parameters. In this paper, a transformer-based generative adversarial network modeling method (T-GAN) is proposed in the THz band, which exploits the advantage of GAN in modeling the complex distribution, and the powerful expressive capability of transformer structure. Experimental results reveal that the distribution of channels generated by the proposed T-GAN method shows good agreement with the original channels in terms of the delay spread and angular spread. Moreover, T-GAN achieves good performance in modeling the power delay angular profile, with 2.18 dB root-mean-square error (RMSE).

==> content/system.tex <==
\section{Problem Formulation}\label{sec_system}
% In this paper, I consider modeling THz SISO channel in an indoor corridor scenario. To model the channel in this scenario, the measurement campaign is conducted in~\cite{yuanbo_icc} with a frequency-domain Vector Network Analyzer (VNA)-based channel sounder. The positions of transmitter and receiver are carefully chosen to characterize the propagation environment in the corridor. Based on the measurement results, 
the channel impulse response (CIR) can be obtained, which can be represented as 
\begin{equation}
    h(\tau) =\sum_{l=0}^{L-1}\alpha_le^{j\phi_l}\delta(\tau-\tau_l),
\end{equation}
where $\tau$ refers to the propagation delay, $\tau_l$ denotes the delay$L$ of the $l$-th multipath, $L$ denotes the number of multi-paths, $\alpha_l$ refers to the path gain and $\phi_l$ represents the phase of the corresponding multi-path. To characterize the channel, power delay profile (PDP) is an important feature, which indicates the dispersion of power over the time delay. It represents the received power with respect to the time of delay in a multi-path channel, which can be extracted from the CIR by
\begin{equation}
    P(\tau) = |h(\tau)|^2.
\end{equation}
Then, the channel modeling problem is to model the distribution of PDP, such that the statistical property of generated distribution of PDP can match the distribution of measurement.









% the 3GPP SISO channel model implemented by Quadriga is considered, while the important statistics of channel are collected from realistic THz measurement campaign~\cite{yuanbo_icc}. 

% I denote the distribution of channel generated by 3GPP model by $P_r$, and the channel samples from the distribution are considered as real channel. The channel modeling problem is formulated as finding the approximate distribution $P_g$, that is close to the real distribution $P_r$. Then, the problem is to minimize the distribution between the two distributions, represented by
% \begin{equation}
%     W(P_r,P_g)=\inf_{\gamma\in \prod(P_r,P_g)}E_{(x,y)\sim\gamma}(\left\|x-y\right\|).
% \end{equation}
% The distance metric chosen is the Earth-Mover (EM) Distance, which can be considered as the optimal cost to transform between two distributions. 



